VideoPoet: A Large Language Model for Zero-Shot Video Generation

We present VideoPoet, a language model capable of synthesizing high-quality video, with matching audio, from a large variety of conditioning signals. VideoPoet employs a decoder-only transformer architecture that processes multimodal inputs -- including images, videos, text, and audio. The training protocol follows that of Large Language Models (LLMs), consisting of two stages: pretraining and task-specific adaptation. During pretraining, VideoPoet incorporates a mixture of multimodal generative objectives within an autoregressive Transformer framework. The pretrained LLM serves as a foundation that can be adapted for a range of video generation tasks. We present empirical results demonstrating the model's state-of-the-art capabilities in zero-shot video generation, specifically highlighting VideoPoet's ability to generate high-fidelity motions. Project page: http://sites.research.google/videopoet/

==> figures/fig_chain_mona_yawn.tex <==
\begin{figure}[ht]
\addtocounter{figure}{-1}
\centering
\begin{subfigure}{0.4\linewidth}
\centering
\videoframe{figures/video_frames/mona_yawn_lores_00001.jpg}
\videoframe{figures/video_frames/mona_yawn_lores_00006.jpg}
\videoframe{figures/video_frames/mona_yawn_lores_00011.jpg}
\videoframe{figures/video_frames/mona_yawn_lores_00017.jpg}
{\textbf{Animated from Still Image}
\ \\
\ \\}
\end{subfigure}
% \vspace{-4mm}


\begin{subfigure}{0.4\linewidth}
\centering
\videoframe{figures/video_frames/mona_yawn_snow_00001.jpg}
\videoframe{figures/video_frames/mona_yawn_snow_00006.jpg}
\videoframe{figures/video_frames/mona_yawn_snow_00011.jpg}
\videoframe{figures/video_frames/mona_yawn_snow_00017.jpg}
{\textbf{Stylized Video} \\
\textbf{Prompt:} An oil painting of a snowman with a red hat opening their mouth to yawn
\ \\}
\end{subfigure}
\captionof{figure}{\textbf{Example of zero-shot video editing via task chaining (text conditioned image-to-video and stylization)} 
%-- the original painting is first animated via a text prompt and then stylized via another text prompt.
}
\label{fig:animate_stylize}
\end{figure}

==> figures/fig_chain_train.tex <==
%\begin{figure*}[h]
\begin{figure}[t]
% \addtocounter{figure}{-1} %Prevent subfigures increasing main figure count  % for some reason, this needed to be commented out to get this figure to have a different number than the preceeding figure.
\centering
% Arc shot
\begin{subfigure}[b]{1.0\linewidth}
%{0.5\textwidth}
\centering
\videoframe{figures/video_frames/train_original_00001.jpg}
\videoframe{figures/video_frames/train_original_00006.jpg}
\videoframe{figures/video_frames/train_original_00011.jpg}
\videoframe{figures/video_frames/train_original_00017.jpg}
%\captionof{figure}{Example of directed camera movement }
%\end{figure}
{\textbf{Original Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}[b]{1.0\linewidth}
\centering
\videoframe{figures/video_frames/train_outpaint_00001.jpg}
\videoframe{figures/video_frames/train_outpaint_00006.jpg}
\videoframe{figures/video_frames/train_outpaint_00011.jpg}
\videoframe{figures/video_frames/train_outpaint_00017.jpg}
{\textbf{Outpainted Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}[b]{1.0\linewidth}
\centering
\videoframe{figures/video_frames/train_food_00001.jpg}
\videoframe{figures/video_frames/train_food_00006.jpg}
\videoframe{figures/video_frames/train_food_00011.jpg}
\videoframe{figures/video_frames/train_food_00017.jpg}
{\textbf{Stylized Video} \\
\textbf{Prompt:} A gingerbread and candy train on a track
\ \\}
\end{subfigure}

\caption{\textbf{Example of zero-shot video editing via task chaining (outpainting and stylization)} -- the original video is first outpainted and then stylized via a text prompt.\lu{We can see a clear artifact in the middle row over the train (white block). This image may raise question.}}
\label{fig:outpaint_stylize}
\end{figure}

==> figures/fig_inpaint_goat_dragon.tex <==
\begin{figure}[t]
\addtocounter{figure}{-1}

\begin{subfigure}{1.0\linewidth}
\centering
\videoframe{figures/video_frames/goat_original_00001.jpg}
\videoframe{figures/video_frames/goat_original_00006.jpg}
\videoframe{figures/video_frames/goat_original_00011.jpg}
\videoframe{figures/video_frames/goat_original_00017.jpg}
{\textbf{Original Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}{1.0\linewidth}
\centering
\videoframe{figures/video_frames/goat_mask_00001.jpg}
\videoframe{figures/video_frames/goat_mask_00006.jpg}
\videoframe{figures/video_frames/goat_mask_00011.jpg}
\videoframe{figures/video_frames/goat_mask_00017.jpg}
{\textbf{Masked Video}
\ \\
\ \\}
\end{subfigure}


\begin{subfigure}{1.0\linewidth}
\centering
\videoframe{figures/video_frames/goat_dragon_00001.jpg}
\videoframe{figures/video_frames/goat_dragon_00006.jpg}
\videoframe{figures/video_frames/goat_dragon_00011.jpg}
\videoframe{figures/video_frames/goat_dragon_00017.jpg}
{\textbf{Inpainted Video from Text Prompt} \\
\textbf{Prompt:} A blue dragon walking along a ridge
\ \\}
\end{subfigure}

\captionof{figure}{
\textbf{\textbf{Example of a task  the model was not explicitly trained for} -- video editing via text conditioned inpainting.}
}
\label{fig:inpainting_dragon_goat}
\end{figure}

==> figures/magvit-v2-config <==
video:
{
  "config": {
    "base_lr": 0.0001,
    "batch_size": "256",
    "data_dtype_str": "float32",
    "dataset_configs": {
      "base_dir": "/readahead/128M",
      "crop_size": "128",
      "dataset_name": "umt_plus_m3",
      "examples_per_subset": {
        "test": "20000",
        "train": "500000000",
        "validation": "20000"
      },
      "frame_rate": "25",
      "label_dir": "/cns/lu-d/home/lijuny/videogvt/datasets",
      "min_resize": "128",
      "num_classes": "0",
      "num_frames": "17",
      "num_test_clips": "1",
      "one_hot_label": false,
      "prefetch_to_device": "2",
      "stride": "1",
      "tables": {
        "test": "/cns/oa-d/home/umt-video-data-access/datasets/umt/25k/raw/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=umt-video-data-access/ttl=30d/latest/umt_25k_tokens@100",
        "train": [
          "/cns/vq-d/home/video-first-data-access/canon/umt500m_rgb_noshot_classfiltered/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=video-first-data-access/ttl=60d/latest/umt500m_rgb_noshot_classfiltered@20000",
          "/placer/prod/home/viva-video-generation/shutterstock/sstk_ml/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=viva-video-generation/latest/sst@99991",
          "/cns/px-d/home/viva-miner/video_miner/faces/rs=6.3/M3/1M/gen/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=viva-miner-faces/ttl=30d/latest/viva_miner_faces_m3_1M_train_gen@80000"
        ],
        "validation": "/cns/oa-d/home/umt-video-data-access/datasets/umt/25k/raw/e=1:kid=73859:mkey=learning_canon_prod_colossus:mdb=umt-video-data-access/ttl=30d/latest/umt_25k_tokens@100"
      },
      "train_sample_weights": [
        0.7,
        0.2,
        0.1
      ],
      "train_stride_overrides": [
        "1",
        "1",
        "3"
      ],
      "zero_centering": false
    },
    "dataset_name": "video_sstable_dataset_multitable",
    "discriminator": {
      "channel_multipliers": [
        "2",
        "4",
        "4",
        "4",
        "4"
      ],
      "downsample": "blur",
      "filters": "128",
      "num_remat_blocks": "2"
    },
    "dtype": "float32",
    "eval": {
      "data_splits": "train,test",
      "enable_frechet_distance": true,
      "enable_inception_score": true,
      "enable_lpips": true,
      "enable_ssim_psnr": true,
      "enable_utilization": true,
      "final_num_repeats": "1",
      "num_examples": "20000"
    },
    "eval_batch_size": "64",
    "eval_from": {
      "checkpoint_path": null,
      "step": null,
      "xm": null
    },
    "experiment_name": "UCF101_VQGAN/3D",
    "image_size": "128",
    "init_from": {
      "inflate_discriminator": false,
      "inflation": "2d->3d/last",
      "xm": [
        "64438688",
        "1"
      ]
    },
    "lax_precision": "default",
    "lecam_weight": 0.001,
    "logging": {
      "checkpoint_kept": "5",
      "checkpoint_steps": "1000",
      "enable_checkpoint": true,
      "log_metric_steps": "200",
      "log_sample_size": "2"
    },
    "lr_configs": {
      "base_learning_rate": 0.0001,
      "factors": "constant * cosine_decay * linear_warmup",
      "learning_rate_schedule": "compound",
      "steps_per_cycle": "1000000",
      "warmup_steps": "5000"
    },
    "model_class": "VQGAN",
    "num_training_steps": "1000000",
    "optimizer": {
      "beta1": 0,
      "beta2": 0.99,
      "d_lr": 0.0001,
      "g_lr": 0.0001,
      "lr": 0.0001
    },
    "perceptual_loss_on_logit": true,
    "perceptual_loss_weight": 0.1,
    "polyak_decay": 0.999,
    "pretrained_image_model": true,
    "rng_seed": "0",
    "sq": {
      "bound_method": "sine",
      "dim_widths": [
        "8",
        "8",
        "4",
        "4",
        "4",
        "4",
        "4",
        "4"
      ],
      "quantize_method": "ste"
    },
    "vqgan": {
      "finetune_decoder": false,
      "finetune_path": "",
      "g_adversarial_loss_weight": 0.1,
      "grad_penalty_cost": 10,
      "gradient_penalty": "r1",
      "loss_type": "non-saturating",
      "model_type": "3D"
    },
    "vqvae": {
      "activation_fn": "swish",
      "architecture": "3dcnn",
      "channel_multipliers": [
        "1",
        "2",
        "2",
        "4"
      ],
      "codebook_size": "262144",
      "commitment_cost": 0.25,
      "conv_downsample": true,
      "custom_conv_padding": "causal_custom",
      "decoder_deep_condition": true,
      "deconv_upsample": false,
      "embedding_dim": "8",
      "entropy_loss_ratio": 0.1,
      "entropy_loss_type": "softmax",
      "entropy_temperature": 0.01,
      "filters": "128",
      "norm_type": "GN_spatial",
      "num_dec_remat_blocks": "2",
      "num_dec_res_blocks": "4",
      "num_enc_remat_blocks": "2",
      "num_enc_res_blocks": "4",
      "reconstruction_loss_weight": 5,
      "temporal_downsample": [
        false,
        true,
        true
      ],
      "upsample": "depth_to_space",
      "vector_quantizer_class": "ScalarQuantizer"
    }
  },
  "eval_while_training": "ACTX__MERGE_VALUE_CONFLICT (go/xm-parameters#work-unit-parameters-and-configurations)",
  "logger_levels": null
}
image:
{
  "config": {
    "base_lr": 0.0001,
    "batch_size": "2048",
    "data_dtype_str": "float32",
    "dataset_configs": {
      "dataset": "imagenet2012",
      "gldm_configs": {
        "alt_text_relevance_high_threshold": 0.7,
        "alt_text_relevance_low_threshold": 0.52,
        "drop_dups": true,
        "drop_empty_text": true,
        "ica_labels_score_threshold": 0.95,
        "ica_labels_to_drop_by": null,
        "ignore_errors": true,
        "max_ica_labels": "3",
        "prefer_alt_text_prob": 1,
        "prepend_ica_labels_prob": 1,
        "random_pali_caption": true,
        "use_proxy": false
      },
      "gldm_ds_names": {
        "train": "webli_v3_tigg_data_v1"
      },
      "image_size": "128",
      "num_classes": "0",
      "pp_eval": "decode|resize_small(128)|central_crop(128)|value_range(0, 1)|copy(\"label\", \"labels\")|keep(\"image\", \"labels\")",
      "pp_train": "keep(\"image\")",
      "prefetch_to_device": "2",
      "shuffle_buffer_size": "10000",
      "text_encoder_name": "dummy",
      "train_split": "train",
      "val_split": "validation"
    },
    "dataset_name": "webli",
    "dataset_type": "image",
    "discriminator": {
      "blur_resample": true,
      "channel_multipliers": [
        "2",
        "4",
        "4",
        "4",
        "4"
      ],
      "filters": "128"
    },
    "dtype": "float32",
    "eval": {
      "data_splits": "train,validation",
      "enable_frechet_distance": false,
      "enable_frechet_image_distance": true,
      "enable_inception_score": false,
      "enable_lpips": true,
      "enable_ssim_psnr": true,
      "enable_utilization": true,
      "final_num_example_multiplier": "5",
      "num_examples": "10000"
    },
    "eval_batch_size": "64",
    "eval_dataset_name": "bit",
    "eval_from": {
      "checkpoint_path": null,
      "step": null,
      "xm": null
    },
    "experiment_name": "ImageNet_VQGAN/2D",
    "image_size": "128",
    "lax_precision": "default",
    "lecam_weight": 0.001,
    "logging": {
      "checkpoint_kept": "5",
      "checkpoint_steps": "10000",
      "enable_checkpoint": true,
      "log_metric_steps": "200",
      "log_sample_size": "8"
    },
    "lr_configs": {
      "base_learning_rate": 0.0001,
      "factors": "constant * cosine_decay * linear_warmup",
      "learning_rate_schedule": "compound",
      "steps_per_cycle": "1000000",
      "warmup_steps": "10000"
    },
    "model_class": "VQGAN",
    "num_training_steps": "1000000",
    "optimizer": {
      "beta1": 0,
      "beta2": 0.99,
      "d_lr": 0.0001,
      "g_lr": 0.0001,
      "lr": 0.0001
    },
    "perceptual_loss_on_logit": true,
    "perceptual_loss_weight": 0.1,
    "polyak_decay": 0.999,
    "pretrained_image_model": true,
    "rng_seed": "0",
    "sq": {
      "bound_method": "sine",
      "dim_widths": [
        "8",
        "8",
        "4",
        "4",
        "4",
        "4",
        "4",
        "4"
      ],
      "quantize_method": "ste"
    },
    "vqgan": {
      "g_adversarial_loss_weight": 0.1,
      "grad_penalty_cost": 10,
      "gradient_penalty": "r1",
      "loss_type": "non-saturating",
      "model_type": "2D"
    },
    "vqvae": {
      "activation_fn": "swish",
      "architecture": "2dcnn",
      "channel_multipliers": [
        "1",
        "2",
        "2",
        "4"
      ],
      "codebook_size": "262144",
      "commitment_cost": 0.25,
      "conv_downsample": true,
      "decoder_deep_condition": true,
      "deconv_upsample": false,
      "embedding_dim": "8",
      "entropy_loss_ratio": 0.1,
      "entropy_loss_type": "softmax",
      "entropy_temperature": 0.01,
      "filters": "128",
      "norm_type": "GN",
      "num_attn_heads": "8",
      "num_dec_res_blocks": "4",
      "num_enc_res_blocks": "4",
      "reconstruction_loss_weight": 5,
      "upsample": "depth_to_space",
      "use_attn": false,
      "vector_quantizer_class": "ScalarQuantizer"
    }
  },
  "eval_while_training": "ACTX__MERGE_VALUE_CONFLICT (go/xm-parameters#work-unit-parameters-and-configurations)",
  "logger_levels": null
}


==> figures/video_samples.tex <==
\begin{figure*}%[!hb]
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_001.png}
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_003.png}
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_004.png}
\videoframe{figures/video_frames/00335_.cfg_4.0.temp_1.0.topp_0.95_a_photorealistic_teddy_bear_is_holding_hands_sr_bins_24_temp_14.5.mp4_006.png}
{\textbf{ Prompt}: A photorealistic teddy bear is holding hands with another teddy bear, walking down 5th avenue when it is raining
\ \\
\ \\}
\end{subfigure}
~
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/mane_00001.jpg}
\videoframe{figures/video_frames/mane_00025.jpg}
\videoframe{figures/video_frames/mane_00030.jpg}
\videoframe{figures/video_frames/mane_00037.jpg}\\
{\textbf{ Prompt}: A lion with a mane made out of yellow dandelion petals roars
\ \\
\ \\
\ \\}
\end{subfigure}
~
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_001.png}
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_003.png}
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_005.png}
\videoframe{figures/video_frames/00104_cfg_3.2.temp_1.0.topp_0.95_a_dog_listening_to_music_with_headphones,_highly_detailed,_cinematic,_high_contrast,_8k_3.gif_006.png}
{\textbf{ Prompt}:  A dog listening to music with headphones, highly detailed, 8k
\ \\
\ \\}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\centering
\videoframe{figures/video_frames/chicken_00001.jpg}
\videoframe{figures/video_frames/chicken_00005.jpg}
\videoframe{figures/video_frames/chicken_00009.jpg}
\videoframe{figures/video_frames/chicken_00012.jpg}
{\textbf{ Prompt}: A chicken lifting weights
\ \\
\ \\
\ \\}
\end{subfigure}

\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00001.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00004.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00008.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00012.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00017.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00023.jpg}
%\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00033.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00038.jpg}
\includegraphics[width=0.12\textwidth]{figures/video_frames/paint_00049.jpg}
{\textbf{ Prompt}: A large blob of exploding splashing rainbow paint, with an apple emerging, 8k
\ \\}
\end{subfigure}
\caption{\textbf{Examples from \modelname{}'s text-to-video generation
results.} Some prompts are edited for clarity.}
\label{fig:video_samples}
\end{figure*}

